Dynamic Multi-Reward Weighting for Multi-Style Controllable Generation

Textual style expresses a diverse set of information, including interpersonal dynamics (e.g., formality) and the author's emotions or attitudes (e.g., disgust). An open question is how language models can be explicitly controlled so that they weave together target styles when generating text: for example, to produce text that is both negative and non-toxic. One approach to such controlled generation is multi-objective reinforcement learning (RL), but how best to combine multiple objectives in a reward function is an open question. In this paper, we investigate various formulations of multi-style rewards, including calibrated outputs from discriminators and dynamic weighting by discriminator gradient magnitudes. We find that our proposed dynamic weighting outperforms static weighting approaches with respect to style control while maintaining linguistic quality, and we explore its effectiveness in 2- and 3-style control.

==> Tables/DiscriminatorEval.tex <==
\begin{table}[]
\begin{tabular}{lll}
              & Sentiment                  & Formality        \\\hline
Training Size & 8540                       & 209118           \\\hline
Testing Size  & 2210                       & 4849             \\\hline
Accuracy      & 51.51\%                    & 89.77\%         
\end{tabular}
\caption{Training Information for LLaMA-based discriminators used.}
\end{table}

==> Tables/EvalTable.tex <==
\begin{table*}[]
\begin{tabular}{llllllllll}
              & \multicolumn{3}{l}{PPLM (deep fusion)} & \multicolumn{3}{l}{SFPPLM}  & \multicolumn{3}{l}{RL} \\\hline
              & Precision    & F1         & Recall     & Precision & F1     & Recall & Precision & F1      & Recall  \\\hline
pos, formal   & 23.00\%      & 6.23\%     & 3.83\%     & 23.40\%   & 6.32\% & 3.90\% & 23.40\%   & 6.32\%  & 3.90\%  \\\hline
pos, informal & 7.60\%       & 2.35\%     & 1.27\%     & 5.40\%    & 1.71\% & 0.90\% & 10.00\%   & 0.33\%  & 0.17\%  \\\hline
neg, ormal   & 9.00\%       & 2.75\%     & 1.50\%     & 9.80\%    & 2.97\% & 1.63\% & 13.20\%   & 3.89\%  & 2.20\%  \\\hline
neg, informal & 6.40\%       & 2.01\%     & 1.07\%     & 7.60\%    & 2.35\% & 1.27\% & 6.40\%    & 2.01\%  & 1.07\%  \\\hline
pos           & 33.80\%      & 16.84\%    & 11.27\%    & -         & -      & -      & 11.60\%   & 6.93\%  & 3.87\%  \\\hline
neg           & 16.60\%      & 9.49\%     & 5.53\%     & -         & -      & -      & 9.80\%    & 5.95\%  & 3.27\%  \\\hline
formal        & 64.00\%      & 39.02\%    & 32.00\%    & -         & -      & -      & 68.80\%   & 47.76\% & 34.40\% \\\hline
informal      & 32.00\%      & 24.24\%    & 16.00\%    & -         & -      & -      & 35.40\%   & 26.14\% & 17.70\%
\end{tabular}
\caption{Evaluation information for various controlled style generation strategies on the evaluation set.}
\end{table*}

==> Tables/domain_RL.tex <==
\begin{table*}[ht]
\centering\small

\begin{tabular}{lccc|ccc|ccc|ccc}
\toprule
\textbf{} & \multicolumn{3}{c}{\textbf{Sem Eval Prompts}} & \multicolumn{3}{c}{\textbf{Tweet Eval}} & \multicolumn{3}{c}{\textbf{Rotten Tomatoes}} & \multicolumn{3}{c}{\textbf{Wikipedia}} \\
\midrule
\textbf{} & \textbf{Sent.} & \textbf{Form.} & \textbf{Both} & \textbf{Sent.} & \textbf{Form.} & \textbf{Both} & \textbf{Sent.} & \textbf{Form.} & \textbf{Both} & \textbf{Sent.} & \textbf{Form.} & \textbf{Both} \\
\midrule
2-Style Models & & & \\
\quad Pos-Formal  & 0.872 & 0.738 & 0.692 & 0.902 & 0.764 & 0.714 & 0.900 & 0.748 & 0.714 & 0.744 & 0.790 & 0.692 \\
\quad Pos-Informal & 0.794 & 0.710 & 0.536 & 0.802 & 0.738 & 0.560 & 0.840 & 0.796 & 0.644 & 0.564 & 0.436 & 0.100 \\
\quad Neg-Formal & 0.732 & 0.572 & 0.398 & 0.720 & 0.606 & 0.398 & 0.820 & 0.512 & 0.404 & 0.450 & 0.598 & 0.118  \\
\quad Neg-Informal & 0.692 & 0.802 & 0.642 & 0.696 & 0.832 & 0.656 & 0.640 & 0.810 & 0.588 & 0.606 & 0.624 & 0.524 \\
\bottomrule
\end{tabular}
\caption{Domain-specific automatic accuracy evaluation of 1- and 2-style models. Prompts from the Wikipedia dataset are particularly challenging.
\dk{can you move this to appendix and make it as a graph plot? I think readers can capture the relative difference of these scores across domains, rather than the actual scores.}
}
\label{tab:precision_domain}
\end{table*}

